A Tight Lower Bound for Counting Hamiltonian Cycles via Matrix Rank

For even $k$, the matchings connectivity matrix $\mathbf{M}_k$ encodes which pairs of perfect matchings on $k$ vertices form a single cycle. Cygan et al. (STOC 2013) showed that the rank of $\mathbf{M}_k$ over $\mathbb{Z}_2$ is $\Theta(\sqrt 2^k)$ and used this to give an $O^*((2+\sqrt{2})^{\mathsf{pw}})$ time algorithm for counting Hamiltonian cycles modulo $2$ on graphs of pathwidth $\mathsf{pw}$. The same authors complemented their algorithm by an essentially tight lower bound under the Strong Exponential Time Hypothesis (SETH). This bound crucially relied on a large permutation submatrix within $\mathbf{M}_k$, which enabled a "pattern propagation" commonly used in previous related lower bounds, as initiated by Lokshtanov et al. (SODA 2011). We present a new technique for a similar pattern propagation when only a black-box lower bound on the asymptotic rank of $\mathbf{M}_k$ is given; no stronger structural insights such as the existence of large permutation submatrices in $\mathbf{M}_k$ are needed. Given appropriate rank bounds, our technique yields lower bounds for counting Hamiltonian cycles (also modulo fixed primes $p$) parameterized by pathwidth. To apply this technique, we prove that the rank of $\mathbf{M}_k$ over the rationals is $4^k / \mathrm{poly}(k)$. We also show that the rank of $\mathbf{M}_k$ over $\mathbb{Z}_p$ is $\Omega(1.97^k)$ for any prime $p\neq 2$ and even $\Omega(2.15^k)$ for some primes. As a consequence, we obtain that Hamiltonian cycles cannot be counted in time $O^*((6-\epsilon)^{\mathsf{pw}})$ for any $\epsilon>0$ unless SETH fails. This bound is tight due to a $O^*(6^{\mathsf{pw}})$ time algorithm by Bodlaender et al. (ICALP 2013). Under SETH, we also obtain that Hamiltonian cycles cannot be counted modulo primes $p\neq 2$ in time $O^*(3.97^\mathsf{pw})$, indicating that the modulus can affect the complexity in intricate ways.

==> collem.tex <==
\usetikzlibrary{calc}
\begin{tikzpicture}[scale=0.45]


\tikzstyle{bn}=[circle,fill=gray,text=white,draw=black]
\tikzstyle{wn}=[circle,fill=white,draw]
\tikzstyle{big2}=[circle,fill=gray,minimum size=1.2cm, draw=black,text=white]
\tikzstyle{mythick}=[line width=4]
\tikzstyle{mydashed}=[dashed, line width=4]
\tikzstyle{mydotted}=[dotted, line width=1]


\foreach \x in {1.95,7}
	\draw[mydotted] (\x,-8) -- (\x,-10);


\foreach \layer/\offset in {1/0, 2/7.5, q/18}
{
\begin{scope}[yshift=-\offset cm]
\coordinate (k\layer) at (1.95, 3.5);
\end{scope}
}

\foreach \i/\offset/\t in {1/0/1, 2/-7.5/2, 3/-10.5/{q-1}} 
{
\node[wn] (y\i) at (-1,\offset) {};
\draw ($(y\i)-(1.2,0)$) node {$y_{\t}'$};
}
\draw[mythick] (y1) -- (k1);
\draw[mythick] (y1) -- (k2);

\draw[mythick] (y2) -- (k2);
\coordinate (tmp) at (1.95,-11.5);
\draw[mythick] (y2) -- ($(y2) !.3! (tmp)$);
\coordinate (tmp2) at (1.95,-7);
\draw[mythick] (y3) -- ($(y3) !.3! (tmp2)$);


\draw[mythick] (y3) -- (kq);


\node[wn] (yq) at (-5,-5.5) {};
\draw[mythick] (yq) edge[bend left=40] (k1);
\draw[mythick] (yq) edge[bend right=40] (kq);
\draw ($(yq)-(1,0)$) node {$y_q'$};


\draw[rounded corners] (3+0.1,6.75) rectangle (3 + 3-0.1, -17.75);
\draw (3 + 1.5, -5) node {$G$};

\foreach \layer/\offset in {1/0, 2/7.5, q/18}
{
\begin{scope}[yshift=-\offset cm]

\draw[rounded corners,fill=white] (1,0.25) rectangle (3-0.1, 6.75);
\draw[rounded corners] (6.1,0.25) rectangle (8, 6.75);
\draw  (k\layer) node {$K_{\beta}^\layer$};
\draw (7.1, 3.5) node {$\hat{K}_{\beta}^\layer$};

\foreach \x in {1,2}
	\foreach \y in {1, ..., 6}
		\node[wn,inner sep=0pt, minimum size=0.3cm] (x\x\y) at (\x * 3, \y) {\tiny $l_{\layer,\y}$};



\end{scope}
}



\end{tikzpicture}

